A Virtual Reality Game to Improve Physical and Cognitive Acuity

We present the Virtual Human Benchmark (VHB) game to evaluate and improve physical and cognitive acuity. VHB simulates in 3D the BATAK lightboard game, which is designed to improve physical reaction and hand-eye coordination, on the \textit{Oculus Rift} and \textit{Quest} headsets. The game comprises the \textit{reaction}, \textit{accumulator} and \textit{sequence} modes; \bj{along} with the \textit{reaction} and \textit{accumulator} modes which mimic BATAK functionalities, the \textit{sequence} mode involves the user repeating a sequence of illuminated targets with increasing complexity to train visual memory and cognitive processing. A first version of the game (VHB v1) was evaluated against the real-world BATAK by 20 users, and their feedback was utilized to improve game design and obtain a second version (VHB v2). Another study to evaluate VHB v2 was conducted with 20 users, whose results confirmed that the deign improvements enhanced game usability and user experience in multiple respects. Also, logging and visualization of performance data such as \textit{reaction time}, \textit{speed between targets} and \textit{completed sequence patterns} provides useful data for coaches/therapists monitoring sports/rehabilitation regimens.

==> alt-text.tex <==
Figure 1: \Description[<An exemplar video from the AFEW-VA dataset, with a negative mood label and a dynamic emotion label.>]{<The image shows a sample video from the AFEW-VA dataset. The video has a negative mood label along with an emotion label which varies depending on the valence values of each frame.>}
Figure 2: \Description[<Figure showing the overview of the proposed mood recognition framework.>]{<The input saamples from the AFEW-VA dataset are trained with a single-branch CNN, with a model-fusion approach, a two-branch CNN and a Teacher-Student Network.>}
Figure 2: \Description[<Figure showing the architecture of the CNN with two branches, trained with mood and delta labels, followed by a multi-layer perceptron.>]{<The architecture of the model fusing both mood and emotional change information. The convolutional layers are shown in blue, the average pooling layers are shown in yellow, the fully connected layer with 512 neurons in red and the last fully connected layer with three neurons in purple.>}
Figure 3: \Description[The left side of the figure shows the architecture of the CNN with two branches trained end-to-end with mood and delta labels, and the right side of the figure shows the architecture of the teacher-student network.]{} 
Figure 4: \Description[Grad-CAM visualisation depicting improved mood prediction in the 2-CNN model.]{The first row of the figure shows an input video sample of Harry Potter with neutral mood label. The second row shows the Grad-CAM output of the 1-CNN model, with the predicted mood label as positive, and a dominant red color over the entire frame in each frame of the sample. The third row is the Grad-CAM output of the 2-CNN model with the heatmap showing yellow-orange color on the face region of the frame, with the predicted mood label as neutral and identical to the ground truth label.}
